VideoPASTA: 7K Preference Pairs That Matter for Video-LLM Alignment

Video-language models (Video-LLMs) excel at understanding video content but struggle with spatial relationships, temporal ordering, and cross-frame continuity. To address these limitations, we introduce VideoPASTA (Preference Alignment with Spatio-Temporal-Cross Frame Adversaries), a framework that enhances Video-LLMs through targeted preference optimization. VideoPASTA trains models to distinguish accurate video representations from carefully crafted adversarial examples that deliberately violate spatial, temporal, or cross-frame relationships. With only 7,020 preference pairs and Direct Preference Optimization, VideoPASTA enables models to learn robust representations that capture fine-grained spatial details and long-range temporal dynamics. Experiments demonstrate that VideoPASTA is model agnostic and significantly improves performance, for example, achieving gains of up to +3.8 percentage points on LongVideoBench, +4.1 on VideoMME, and +4.0 on MVBench, when applied to various state-of-the-art Video-LLMs. These results demonstrate that targeted alignment, rather than massive pretraining or architectural modifications, effectively addresses core video-language challenges. Notably, VideoPASTA achieves these improvements without any human annotation or captioning, relying solely on 32-frame sampling. This efficiency makes our approach a scalable plug-and-play solution that seamlessly integrates with existing models while preserving their original capabilities.

==> figures/pasta_scaling.tex <==

\begin{figure*}[t]
    \centering
    \begin{tabular}{ccc}
        \includegraphics[width=0.30\textwidth]{images/videopasta_mlvu.pdf} &
        \includegraphics[width=0.30\textwidth]{images/videopasta_longvideobench.pdf} &
        \includegraphics[width=0.30\textwidth]{images/videopasta_videomme.pdf} \\
        (a) MLVU & (b) LongVideoBench & (c) VideoMME
    \end{tabular}
\caption{\textbf{Impact of preference data size on model performance}. We evaluate our model's performance across three benchmarks while varying the number of preference pairs used for training.}

    \label{fig:size_vs_benchmark}
\end{figure*}

==> tables/ablation_agnostic.tex <==
\begin{table}[t]
   \centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lccc}
\toprule  
\textbf{Model} & \textbf{MLVU} & \textbf{LongVideoBench} & \textbf{VideoMME} \\
\midrule
VideoLLaVA~\cite{videollava} & 47.3 & 39.1 & 39.9 \\
\rowcolor{cyan!15} + \textbf{\modelname} \hspace{-0.2em}~\raisebox{-0.2ex} {\includegraphics[height=1em]{images/pasta.pdf}} & \textbf{50.2}$_{\mathbf{+6.13\%}}$ & \textbf{42.4}$_{\mathbf{+8.44\%}}$ & \textbf{40.5}$_{\mathbf{+1.50\%}}$ \\
\midrule
LLaVA-NeXT-Interleave~\cite{liLLaVANeXTInterleaveTacklingMultiimage2024} & 52.5 & 44.8 & 48.3 \\
\rowcolor{cyan!15}+  \textbf{\modelname} \hspace{-0.2em}~\raisebox{-0.2ex} {\includegraphics[height=1em]{images/pasta.pdf}} & \textbf{54.0}$_{\mathbf{+2.85\%}}$ & \textbf{45.5}$_{\mathbf{+1.56\%}}$ & \textbf{49.9}$_{\mathbf{+3.31\%}}$ \\
\midrule
LLaVA-OneVision~\citep{llavaonevision} & 64.9 & 56.3 & 58.2 \\
\rowcolor{cyan!15}+  \textbf{\modelname} \hspace{-0.2em}~\raisebox{-0.2ex} {\includegraphics[height=1em]{images/pasta.pdf}} & \textbf{66.3}$_{\mathbf{+2.16\%}}$ & \textbf{56.8}$_{\mathbf{+0.89\%}}$ & \textbf{60.9}$_{\mathbf{+4.64\%}}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Model-agnostic improvements from \modelname}.}
\label{tab:model_agnostic}

\end{table}

==> tables/ablation_frame_sampling.tex <==

\begin{table}[!t]
  \centering
  \begin{adjustbox}{width=\linewidth,center}
    \begin{tabular}{lccc}
      \toprule  
      \textbf{Frame Sampling} & \textbf{MLVU} & \textbf{LongVideoBench} & \textbf{VideoMME} \\
      \midrule
      \ \ 32:32 & 68.7 & 60.8 & 62.4 \\
      \ \ 16:16 & 68.6 & 60.7 & 62.3 \\
      \midrule
      \ \ 32:8 & 69.0 & 61.2 & 63.5 \\
      \ \ 16:4 & 68.9 & 61.0 & 63.2 \\
      \midrule
      \ \ \textbf{32:1 (Ours)} & \textbf{69.2} & \textbf{61.5} & \textbf{64.1} \\
      \ \ 16:1 & 69.0 & 61.3 & 63.7 \\
      \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{\textbf{Effect of frame sampling rates.} Best results in \textbf{bold}.}

  \label{tab:frame_sampling}
\end{table}


==> tables/ablation_negatives.tex <==
\begin{table}[t]
 \centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lccc}
\toprule  
\textbf{Adversarial Examples per} & \textbf{MLVU} & \textbf{LongVideoBench} & \textbf{VideoMME} \\
\textbf{Aligned Sample} & & & \\
\midrule
1 & 67.5 & 58.8 & 62.3 \\
2 & 68.4 & 60.2 & 63.2 \\
\textbf{3 (Ours)} & \textbf{69.2} & \textbf{61.5} & \textbf{64.1} \\
4 & 68.9 & 61.2 & 63.8 \\
5 & 68.7 & 61.0 & 63.6 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Effect of the number of adversarial examples per aligned sample.} Performance peaks at 3 adversarial examples, matching our three targeted failure modes (spatial, temporal, and cross-frame misalignment).}
\label{tab:num_negatives}
\end{table}

==> tables/all_model_agnostic.tex <==
\begin{table}[t]
  \centering
\begin{adjustbox}{width=\linewidth,center}
\fontsize{5.5pt}{6.5pt}\selectfont
\setlength{\tabcolsep}{0.8pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{lcccccccc}
\toprule  
\textbf{Model} & \textbf{TC} & \textbf{PT} & \textbf{NQA} & \textbf{MVB} & \textbf{VG} & \textbf{MLVU} & \textbf{LVB} & \textbf{VMME} \\
\midrule
VideoLLaVA & 66.4 & 67.9 & 74.2 & 58.6 & 24.3 & 47.3 & 39.1 & 39.9 \\
+ Hound-DPO & \na & \na & \na & \na & \na & \na & \na & \na \\
+ TPO & \na & \na & \na & \na & \na & \na & \na & \na \\
+ \modelname\! \raisebox{-0.2ex}{\includegraphics[height=0.7em]{images/pasta.pdf}} &\na & \na & \na & \na & \na & \textbf{50.2}$_{\mathbf{+6.1\%}}$ & \textbf{42.4}$_{\mathbf{+8.4\%}}$ & \textbf{40.5}$_{\mathbf{+1.5\%}}$ \\
\midrule
LLaVA-NeXT-I & 54.1 & 51.2 & 67.0 & 46.5 & 15.2 & 52.5 & 44.8 & 48.3 \\
+ Hound-DPO & \na & \na & \na & \na & \na & \na & \na & \na \\
+ TPO & \na & \na & \na & \na & \na & \na & \na & \na \\
+ \modelname\! \raisebox{-0.2ex}{\includegraphics[height=0.7em]{images/pasta.pdf}} & \na & \na & \na & \na & \na & \textbf{54.0}$_{\mathbf{+2.9\%}}$ & \textbf{45.5}$_{\mathbf{+1.6\%}}$ & \textbf{49.9}$_{\mathbf{+3.3\%}}$ \\
\midrule
LLaVA-OneVision & 64.5 & 57.1 & 79.3 & 56.7 & 25.0 & 64.9 & 56.3 & 58.2 \\
+ Hound-DPO & \na & \na & \na & \na & \na & \na & \na & \na \\
+ TPO & \na & \na & \na & \na & \na & \na & \na & \na \\
+ \modelname\! \raisebox{-0.2ex}{\includegraphics[height=0.7em]{images/pasta.pdf}} & \na & \na & \na & \na & \na & \textbf{66.3}$_{\mathbf{+2.2\%}}$ & \textbf{56.8}$_{\mathbf{+0.9\%}}$ & \textbf{60.9}$_{\mathbf{+4.6\%}}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Comprehensive.}}
\label{tab:all_model_agnostic}
\end{table}

==> tables/cross_model.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\fontsize{6pt}{3pt}\selectfont
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} & \textbf{TC} & \textbf{PT} & \textbf{NQA} & \textbf{MVB} & \textbf{VG} & \textbf{MLVU} & \textbf{LVB} & \textbf{VMME} \\
\midrule
Qwen2.5-VL + InternVL-pref & \na & \na & \na & \na & \na & \na & \na & \na \\
InternVL2.5 + Qwen-pref & \na & \na & \na & \na & \na & \na & \na & \na \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Cross-model preference transfer evaluation}. }
\label{tab:cross_model_preferences}
\end{table}

==> tables/qwen_params.tex <==
\begin{table*}[!t]
\centering
\begin{adjustbox}{width=\textwidth,center}
\setlength{\tabcolsep}{1.5pt} 
\renewcommand{\arraystretch}{1.2} 
\fontsize{5.5pt}{6.5pt}\selectfont
\begin{tabular}{lccccccc}
\toprule
\textbf{Configuration} & \textbf{TempCompass} & \textbf{Perception Test} & \textbf{NeXTQA} & \textbf{MVBench} & \textbf{MLVU} & \textbf{LongVideoBench} & \textbf{VideoMME} \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{DPO Weight Ratio ($\alpha$:$\beta$:$\gamma$) for Qwen2.5-VL}} \\
\midrule
1:1:1 (Equal Weights) & \na & \na & \na & \na & \na & \na & \na \\
3:1:1 (Spatial Focus) & \na & \na & \na & \na & \na & \na & \na \\
1:3:1 (Temporal Focus) & \na & \na & \na & \na & \na & \na & \na \\
1:1:3 (Cross-Frame Focus) & \na & \na & \na & \na & \na & \na & \na \\
\textbf{0.4:0.4:0.2 (Ours)} & \textbf{72.3} & \textbf{69.4} & \textbf{77.3} & \textbf{66.3} & \textbf{69.2} & \textbf{61.5} & \textbf{64.1} \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Adversarial Examples per Aligned Sample (Qwen2.5-VL)}} \\
\midrule
1 & \na & \na & \na & \na & 67.5 & 58.8 & 62.3 \\
2 & \na & \na & \na & \na & 68.4 & 60.2 & 63.2 \\
\textbf{3 (Ours)} & \na & \na & \na & \na & \textbf{69.2} & \textbf{61.5} & \textbf{64.1} \\
4 & \na & \na & \na & \na & 68.9 & 61.2 & 63.8 \\
5 & \na & \na & \na & \na & 68.7 & 61.0 & 63.6 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Frame Sampling (Aligned:Adversarial) for Qwen2.5-VL}} \\
\midrule
32:32 & \na & \na & \na & \na & 68.7 & 60.8 & 62.4 \\
16:16 & \na & \na & \na & \na & 68.6 & 60.7 & 62.3 \\
32:8  & \na & \na & \na & \na & 69.0 & 61.2 & 63.5 \\
16:4  & \na & \na & \na & \na & 68.9 & 61.0 & 63.2 \\
\textbf{32:1 (Ours)} & \na & \na & \na & \na & \textbf{69.2} & \textbf{61.5} & \textbf{64.1} \\
16:1  & \na & \na & \na & \na & 69.0 & 61.3 & 63.7 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Image Resolution Ablation (Qwen2.5-VL)}} \\
\midrule
MIN=4$\times$28$\times$28, MAX=64$\times$28$\times$28 & \na & \na & \na  & \na & \na & \na & \na \\
MIN=4$\times$28$\times$28, MAX=96$\times$28$\times$28 & \na & \na & \na & \na & \na & \na & \na \\
MIN=4$\times$28$\times$28, MAX=128$\times$28$\times$28 & 72.3 & 69.4 & 77.3 & 66.3  & 69.2 & 61.5 & 64.1 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Video Resolution Ablation (Qwen2.5-VL)}} \\
\midrule
VID\_MIN=32$\times$28$\times$28, VID\_MAX=32$\times$28$\times$28 & \na & \na &  \na & \na & \na & \na & \na \\
VID\_MIN=48$\times$28$\times$28, VID\_MAX=48$\times$28$\times$28 & \na & \na & \na & \na & \na & \na & \na \\
VID\_MIN=64$\times$28$\times$28, VID\_MAX=64$\times$28$\times$28 & 72.3 & 69.4 & 77.3 & 66.3  & 69.2 & 61.5 & 64.1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Comprehensive Ablation Studies for \modelname{} on Qwen2.5-VL.} This table details the impact of DPO weight ratios ($\alpha:\beta:\gamma$), the number of adversarial examples per aligned sample, frame sampling strategies (aligned:adversarial frames), and Qwen specific image/video resolutions. Our chosen configurations are in \textbf{bold}.}
\label{tab:qwen_params_comprehensive}
\end{table*}

==> tables/self_vs_internvl.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\fontsize{6pt}{3pt}\selectfont
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{lccccccccc}
\toprule
\textbf{Model} & \textbf{TC} & \textbf{PT} & \textbf{NQA} & \textbf{MVB} & \textbf{VG} & \textbf{MLVU} & \textbf{LVB} & \textbf{VMME} \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{c}{\textit{Baselines}} \\
\midrule
Qwen2.5-VL-7B & 71.7 & 68.6 & 75.8 & 65.2 & 27.9 & 68.7 & 60.7 & 62.2 \\
InternVL2.5-8B & 68.3 & 62.2 & 77.0 & 69.8 & 29.4 & 59.5 & 52.9 & 57.9  \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{c}{\textit{VideoPASTA w/o InternVL2.5-38B}} \\
\midrule
Qwen2.5-VL-7B & \na & \na & \na & \na & \na & \na & \na & \na \\
InternVL2.5-8B & \na & \na & \na & \na & \na & \na & \na & \na \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{c}{\textit{VideoPASTA with InternVL2.5-38B}} \\
\midrule
Qwen2.5-VL-7B & 72.3 &
 69.4 &
 77.3 &
 66.3 &
 28.3 &
 69.2 &
 61.5 &
 64.1 \\
InternVL2.5-8B & \na & \na & \na & \na & \na & \na & \na & \na \\
\midrule
\rowcolor{cyan!15}InternVL2.5-38B & \na & \na & \na & \na & \na & 70.8 & 63.4 & \na \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Comparison of}.}
\label{tab:self_vs_internvl}
\end{table}

==> tables/targeted_alignment.tex <==
\begin{table}[t]
   \centering
\begin{adjustbox}{width=\columnwidth,center}
\fontsize{6pt}{3pt}\selectfont
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{lcccc}
\toprule  
\textbf{Model} & \textbf{Temporal} & \textbf{Spatial} & \textbf{Action} & \textbf{Object} \\
\midrule
Qwen2.5-VL & 35.0 & 63.6 & 54.0 & 55.9 \\
\midrule
w/ Temporal Only & 44.0 & 67.1 & 49.2 & 51.3 \\
w/ Spatial Only & 40.1 & 74.8 & 55.0 & 55.4 \\
w/ Cross-Frame Only & 43.3 & 66.8 & 54.9 & 57.2 \\
w/ TPO & \na & \na & \na & \na \\
w/ Hound-DPO & \na & \na & \na & \na \\
\midrule
\textbf{Full Model} & 
\textbf{45.2}$_{\mathbf{+29.14\%}}$ & 
\textbf{78.6}$_{\mathbf{+23.58\%}}$ & 
\textbf{56.1}$_{\mathbf{+3.89\%}}$ & 
\textbf{58.4}$_{\mathbf{+4.47\%}}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Effect of each targeted failure mode on VideoMME}.}
\label{tab:targeted_alignment}
\end{table}
